Fab Four: When John and George play gravitation and cosmology

Scalar-tensor theories of gravitation have recently regained a great interest after the discovery of the Chameleon mechanism and of the Galileon models. The former allows, in principle, to reconcile the presence of cosmological scalar fields with the constraints from experiments at the Solar System scale. The latter open up the possibility of building inflationary models that, among other things, do not need ad hoc potentials. Further generalizations have finally led to the most general tensor-scalar theory, recently dubbed the "Fab Four", with only first and second order derivatives of the fields in the equations of motion and that self-tune to a vanishing cosmological constant. This model has a very rich phenomenology that needs to be explored and confronted with experimental data in order to constrain a very large parameter space. In this paper, we present some results regarding a subset of the theory named "John", which corresponds to a non-minimal derivative coupling between the scalar field and the Einstein tensor in the action. We show that this coupling gives rise to an inflationary model with very unnatural initial conditions. Thus, we include a non-minimal, but non-derivative, coupling between scalar field and Ricci scalar, a term named "George" in the Fab Four terminology. In this way, we find a more sensible inflationary model, and, by performing a post-newtonian expansion of spherically symmetric solutions, we derive the set of equations that constrain the parameter space with data from experiments in the solar system.

==> section1.tex <==
\section{Introduction}

\noindent The Galileon theory has recently emerged as an effective theoretical realization of the Dvali-Gabadaze-Porrati model (DGP)  \cite{Nicolis:2008in}. The subsequent developments eventually led to the definition of the most general second order scalar-tensor theory that includes, besides the usual terms of scalar-tensor or $f(R)$ theories (as in, e.g. \cite{PhysRevD.1.3209, Damour:1992we, Damour:1993id, Perrotta:1999am, Nojiri:2003ft, Chiba:2003ir, Capozziello:2007ec, Sotiriou:2008rp, Clifton:2011jh}), also non-minimal derivative couplings to the curvature \cite{Deffayet:2009wt, Deffayet:2011gz, Deffayet:2009mn}. This general theory, explored for the first time by the pioneering work of Horndeski many years ago \cite{Horndeski}, provides a wide framework that virtually encompasses all scalar models analyzed so far in the literature.

One interesting aspect of the non-linearities of the scalar sector is that they trigger the Vainshtein mechanism that makes possible to build viable cosmological models with sufficiently small effects at local scales to evade Solar System constraints.  Therefore, we have at hand an interesting alternative to chameleons \cite{Khoury:2003rn}, in which the parameter space for local gravity does not overlap with the one  allowed by  cosmic acceleration, as recently shown in \cite{Hees:2011mu}. In addition, inflationary phases are permitted without the introduction of ad hoc scalar potentials, making these models more ``natural''.
Non-linearities are also responsible for new phenomena in the dark sector including, for instance, sub/superluminality and/or effective violation of the Null Energy Condition, thus allowing for a stable and well-defined phantom-like phase \cite{Babichev:2007dw, Creminelli:2010ba, Babichev:2010kj, Deffayet:2010qz}. Generally speaking, the Galileon model has opened the way to new models for cosmology, including inflationary or late-accelerated ones \cite{Chow:2009fm, Charmousis:2011bf, Kobayashi:2011nu, Tsujikawa:2012mk}. In fact, almost all sort of cosmological scenarios are possible depending on which Galileon model is chosen, see e.g. \cite{Saridakis:2010mf}.

In this paper, we first focus on a subclass of models dubbed ``purely kinetic gravity" \cite{Sushkov:2009hk, Saridakis:2010mf, Gubitosi:2011sg, Germani:2010hd}, or also similar to ``John Lagrangian" in the ``Fab Four's'' terminology\footnote{ Note that in the Fab Four Lagrangian, the scalar field has no standard kinetic term. It propagates however, via its derivative coupling to the curvature tensors.} \cite{Charmousis:2011bf, Charmousis:2011ea}. More generally speaking, it is a special case of the very general Galileon class considered in \cite{Kobayashi:2011nu}. We mostly investigate the inflationary phase and its naturalness, taking into account no-ghost constraints and causality conditions. In a next step, a generalization of the theory including a coupling of the scalar field to the matter -- via, in the Jordan frame, a Brans-Dicke like coupling to the scalar curvature, is introduced. The analysis of the inflationary phase is then reconducted in such a more realistic theory, while a preliminary analysis of solar system constraints is discussed.

We begin in Sec.~\ref{sec2} with a review of John's equations of motion in a flat and empty Universe. We then complete the analysis made in \cite{Sushkov:2009hk} by computing the number of e-folds  in Sec. \ref{sec2b}. We show that a kinetically driven inflationary phase requires highly transplanckian values for the initial field velocity, which rule out the model. Moreover, in Sec.~\ref{sec2c} we provide for a detailed analysis of the no-ghost and causality conditions during cosmic evolution, and we show that the theory becomes acausal for such transplanckian values unless the coupling constant is vanishingly small or if the initial Hubble constant is transplanckian. In passing, we prove that some claims made in the literature regarding the sign of the coupling constant are wrong. We argue that this model is to be discarded also because there are no reasons why the scalar field should be generated at all in the first place. This is particularly clear in an astrophysical context where the theory is forced to reduce to pure GR ($\phi=0$), when the same equations are solved inside a compact body.

In Sec.~\ref{sec3}, we  thus extend our considerations to a more general model, in which we also include a coupling of the scalar field to the Ricci scalar. This corresponds to the ``John plus George'' combination in the Fab Four's terminology. We derive and study numerically the equations of motion for the matter-free cosmological background as well as the no-ghosts and causality conditions. We find that inflation is possible provided both coupling constants are positive. In Sec.~\ref{sec3c} we derive the field equations in spherical and static symmetry, and we briefly sketch how to put some constraints on the parameter space using Solar System tests. We conclude in Section IV with some remarks and perspectives.


==> section2d.tex <==
\subsection{Discussion}
\label{sec2d}
We have established that kinetically driven inflation in the Galileon theory involving the simplest coupling to Einstein tensor is not viable. It requires unnatural transplanckian values for the initial velocity of the field, which, in turn, implies various instabilities. 

This model has anyway another serious drawback. In the absence of any direct coupling to the Ricci scalar, there is no reason why the scalar field  should be generated at all (even in presence of cosmological matter fluid). In other words, $\phi =0$ is always a solution in this class of models, whatever the matter content is. At local scales, this problem appears in the following way. We checked numerically that a relativistic star (with flat asymptotic conditions) must be described by pure GR, i.e.  $\phi=0$ for all $r$ is the only solution that is regular at the center of the star. To conclude, the model considered so far is trivial in the sense that it cannot be different than GR, except if one imposes non-vanishing initial conditions for the scalar field at early times.

This acts as a leitmotiv for a more realistic model, studied in the next section, where we add to the Lagrangian a direct coupling to the Ricci scalar: $F(\phi) R$, namely the "George" term in the Fab Four terminology, and where only a particular function $F$ will be analyzed here.
